RNNFast: An Accelerator for Recurrent Neural Networks Using Domain Wall Memory

Recurrent Neural Networks (RNNs) are an important class of neural networks designed to retain and incorporate context into current decisions. RNNs are particularly well suited for machine learning problems in which context is important, such as speech recognition and language translation. This work presents RNNFast, a hardware accelerator for RNNs that leverages an emerging class of non-volatile memory called domain-wall memory (DWM). We show that DWM is very well suited for RNN acceleration due to its very high density and low read/write energy. At the same time, the sequential nature of input/weight processing of RNNs mitigates one of the downsides of DWM, which is the linear (rather than constant) data access time.RNNFast is very efficient and highly scalable, with flexible mapping of logical neurons to RNN hardware blocks. The basic hardware primitive, the RNN processing element (PE) includes custom DWM-based multiplication, sigmoid and tanh units for high density and low-energy. The accelerator is designed to minimize data movement by closely interleaving DWM storage and computation. We compare our design with a state-of-the-art GPGPU and find21.8x higher performance with70x lower energy

==> changes.tex <==
We thank the reviewers for their time and feedback! Below we summarize changes made to the manuscript. All changes are highlighted in yellow in the manuscript. 

\section*{Summary of Changes in Revised Version}
\begin{itemize}
\item \textbf{Referee 3}:
\textcolor{blue}{\textit{ In ReRAM based accelerators, ISAAC is proposed in 2016, which is relatively old. The authors should compare the proposed method with other the most recent state-of-the-arts, such as PUMA.}}

\hfill

We have updated the evaluation section of the paper to include a comparison with the PUMA accelerator presented in \cite{ankit2019puma}. The authors of PUMA released a simulator that we use to run our benchmarks. We also consulted with the authors to make sure our methodology was sound. We found the performance of PUMA to be lower than that of ISAAC-RNN (our implementation of ISAAC for RNN networks). This result was expected since PUMA is designed to be much more general, and support both CNNs and RNNs. This generality comes at the cost of higher overhead relative to ISAAC-RNN. In \cite{ankit2019puma} the authors compare to the original ISAAC for CNN workloads and similarly find ISAAC to perform better that PUMA for those benchmarks. RNNFast is even more efficient, primarily due to the high density and low power of the DWM cell. RNNFast consumes about 25\% the energy of PUMA.  

%We find RNNFast consume $4\times$ less energy than PUMA.

% PUMA does not show better performance than GPU consistently. GPU has better performance for networks with hidden size which are power of 2. In other cases PUMA performs better. Overall PUMA tends to have better performance than GPU for larger networks specially for multi-layer networks (seq2seq) where PUMA benefits from pipelining through layers. GPU shows sub-linear runtime increase regarding the number of time steps, therefore the D-speech with 1500 time-steps shows similar runtime in both GPU and PUMA. It is notable to mention that we used Deepbench to run GPU benchmarks which only measures purely running RNN layers without inefficiencies of running models over frameworks like Torch7. Thus Those are the best runtimes we can get from GPU. Also PUMA reported lower throughput than ISAAC. The ISAAC-RNN shows better speedup than PUMA. RNNFast shows better performance than PUMA in all benhcmarks.
%PUMA energy consumption is much lower than GPU but as expected is not better that ISAAC design. RNNFast consume $4\times$ less energy than PUMA.

\hfill

\textcolor{blue}{\textit{Regarding the overall accuracy. RNNs are more sensitive compared to CNNs when we run one RNN layer with thousands of time steps. The authors mentioned that "A great body of previous works 6-10 showed that for training and especially inference as few as 8 bits of precision are sufficient to have virtually no impact on the accuracy of neural networks". For CNNs, 8-bit might be sufficient to have virtually no impact on the accuracy. But for RNNs, 8-bit may cause severe accuracy degradation. Have the authors investigated the error-accumulation in RNNs with significant amount of time steps.}}

\hfill

We have not directly examined the effect of representation precision on the output accuracy of RNNs. Since this has been explored in prior RNN designs, we considered this aspect to be out of scope for this work. In our design we used 16 bit fixed point precision. This is consistent with prior work on RNN accelerators \cite{Ferreira_16ReConfig, han2017ese,ankit2019puma}. \cite{chang2015recurrent} used the fixed point Q8.8  data format. Their measured error rate does not appear to significantly accumulate over multiple time steps and it stabilizes at 3.9\% for $c_t$ and 2.9\% for $h_t$. Other works have shown some RNN designs can use even lower precision. For instance, %\cite{han2017ese} used 12 bits and 
\cite{shin2016fixed} investigated the impact of fixed-point precision on RNNs used for phoneme recognition and language modeling. They showed that for phoneme recognition most weights can be represented with 3 bits, while language modeling needs 5 or 6 bits for achieving accuracy close to floating-point representation. %Also \cite{li2018rnn} reported <0.1\% accuracy degradation for input/weight quantization to 12 bits. %\cite{li2018fpga} even used 8-bit fixed point with limited accuracy loss. 




\end{itemize}
\newpage

==> definitions.tex <==
\def\degrees{$^{\mbox{\rm \,\footnotesize o}}$C}	%% Celsius
\def\Ileak{I_{\mbox{\rm \footnotesize leak}}}		%% leakage current
\def\Ileakz{I^0_{\mbox{\rm \footnotesize leak}}}	%% leakage current 0
\def\Pleak{P_{\mbox{\rm \footnotesize leak}}}		%% leakage power
\def\Pleakz{P^0_{\mbox{\rm \footnotesize leak}}}	%% leakage power 0
\def\Vth{V_{\mbox{\rm \footnotesize th}}}		%% Vth
\def\Vdd{V_{\mbox{\rm \footnotesize dd}}}		%% Vdd
\def\Leff{L_{\mbox{\rm \footnotesize eff}}}		%% Leff
\def\dVth{\Delta V_{\mbox{\rm \footnotesize th}}}	%% Delta Vth
\def\Vthz{V^0_{\mbox{\rm \footnotesize th}}}		%% Vth0
\def\fmax{f_{\mbox{\rm \footnotesize max}}}		%% fmax
\def\fmaxz{f^0_{\mbox{\rm \footnotesize max}}}		%% fmax0
\def\mean#1{\mbox{\rm E}[ #1 ]}				%% E[...]
\def\Ncp{N_{\mbox{\rm \footnotesize cp}}}		%% number of c.p.
\def\ncp{n_{\mbox{\rm \footnotesize cp}}}		%% depth of c.p.
\def\sncp{n_{\mbox{\rm \scriptsize cp}}}		%% depth of c.p. (small)
\def\Tcp{T_{\mbox{\rm \footnotesize cp}}}		%% delay of c.p.
\def\maxTcp{\max\{ \Tcp \}}				%% max of Tcp
\def\PDF{\mbox{\rm PDF}}				%% prob density func
\def\CDF{\mbox{\rm CDF}}				%% cumulative density func
\def\D2D{\mbox{\rm \scriptsize D2D}}
\def\WID{\mbox{\rm \scriptsize WID}}
\def\Small{\small}

\def\hsuisov{\mathrm{HSU}_{\mathrm{isoV}}}
\def\hsuisop{\mathrm{HSU}_{\mathrm{isoP}}}

%%\newcommand{\ie}{i.e.\ }
%%\newcommand{\eg}{e.g.\ }
%%\newcommand{\varlt}{\stackrel{_\circ}{<}}
\newcommand{\fixme}[1]{\textbf{***FIXME: #1***}}
%%\newcommand{\comment}[1]{{}}

\makeatletter
\def\bstctlcite{\@ifnextchar[{\@bstctlcite}{\@bstctlcite[@auxout]}}
\def\@bstctlcite[#1]#2{\@bsphack
 \@for\@citeb:=#2\do{%
   \edef\@citeb{\expandafter\@firstofone\@citeb}%
   \if@filesw\immediate\write\csname #1\endcsname{\string\citation{\@citeb}}\fi}%
 \@esphack}
\makeatother


==> dwm_mac.tex <==
\subsection{Domain Wall Multiplier}

The RNNFast computational fabric relies on a large number of multipliers. To reduce their area and energy consumption we use a DWM-based multiplier in our design. Recent work \cite{luo_aspdac2016, wang_nanotech2015, Huang_TCS_15} has shown DWM-based ALU designs that achieve 70-80\% area reduction and 50\% energy savings without sacrificing performance. 

%Note that latency of DWM-based adder is still in $\sim$ps range while eliminating transfer time which consumes $\sim$ns. 

We extend the DWM-based multiplier in \cite{luo_aspdac2016} with improvements and optimizations specific to our application. The multiplier uses the radix-4 Booth algorithm, which reduces the number of partial results and accumulation by a factor of two compared to radix-2. The DWM-based implementation of radix-4 requires only a few basic operations. These are multiplication by $\pm2$, $\pm1$ and 0, along with addition, which are accomplished through XOR and majority functions. Instead of the summation logic used in \cite{luo_aspdac2016} we use a negating circuit and an XOR function that uses stacked DWM \cite{wang_nanotech2015}. This saves two transistors per bit. Transistors dominate the area of the DWM adder, so the savings are significant. 

%\begin{figure}
%\centering
%\includegraphics[width=0.65\linewidth,trim = 0 0 0 0 0]{figs/Adder2.pdf}
%\caption{1-bit DWM-based adder.}\label{Fig.:Adder}
%\end{figure}

\begin{comment}
%In radix-4 Booth algorithm, we consider the bits in blocks of three, such that each block overlaps the previous block by one bit. Therefore 
A $3\times8$ decoder is needed to implement radix-4 Booth algorithm. 
%Using radix-4 booth algorithm is better fit for our design over radix 2 and radix 8 implementations. 
Radix-4 by using racetrack memory only requires 7 simple operations. These operations are multiplying by $\pm2$, $\pm1$ and 0 which can be done with maximum one shift in racetrack memory. We use the negating circuit presented in \cite{luo_aspdac2016} to supply -1,-2 operation. Furthermore, when using racetrack, addition can be naturally accomplished through XOR and majority functions.
In other words, by stacking the memory domain that is separated by domain wall and performing one read, we can obtain XOR and majority functions out of it
\end{comment}


\begin{comment}
\begin{table}[h]
\small
\centering

\begin{tabular}{|l|l|l|l|l|}
\hline
Cin & A & B & Sum & Operation\\
\hline
0 & 0 & 0 & 0 & shift A \\
\hline
0 & 0 & 1 & 1 & shift A \\
\hline
0 & 1 & 0 & 1 & flip A \\
\hline
0 & 1 & 1 & 0 & flip A \\
\hline
1 & 0 & 0 & 1 & flip A \\
\hline
1 & 0 & 1 & 0 & flip A \\
\hline
1 & 1 & 0 & 0 & shift A \\
\hline
1 & 1 & 1 & 1 & shift A \\
\hline
\end{tabular}

\caption{Truth table for DWM multiplier.}
\label{tab:truth_table}
\end{table}
\end{comment}


\begin{comment}
We slightly modified the booth multiplier pipeline presented in previous work to better fit our accelerator design and save number of transistors which are main area contributor in DWM-basd adders.
Figure~\ref{Fig.:Adder} shows a single bit adder. It consists of majority function for the
carry out computation. Instead of summation logic we use a negating circuit \cite{luo_aspdac2016} and an XOR function of stacked domain wall memory \cite{wang_nanotech2015} in order to implement the sum logic. Based on table \ref{tab:truth_table} the output of (Cin XOR B) decides whether the sum is equal to $A$ or $\bar{A}$. We use this logic in order to modify the sum function to just shift A value into sum or overwrite the negative value of A and then triggers shift operation. The next adder will read from where we build a pipeline of adders over single racetrack in our adder hierarchy. Adders shift forward the the computed $C_{out}$ with $C_{in}$ in order to use for next step computation.

\end{comment}


\begin{comment}
Figure~\ref{Fig.:MAC} shows an 8-bit version of the multiplier we used for the MAC engine inside each PE. An interleaved multiplier has controllers which contain decoders for radix-4 booth algorithm. The multiplicand is within a single racetrack. Each controller modifies appropriate changes on the incoming bit of multiplicand and sends it the tree based structure of adders which are formed in a pipelines as is shown in Figure~\ref{Fig.:Adder}. Based on which segment of multiplier is the input of controllers, controllers injecting whether zero values or modified multiplicand incoming bit to the adders hierarchy. This multiplier is extensible to enable higher bits length by just duplicating the 8-bit multiplier and providing the adequate number of adders to the adder hierarchy. The final result is accumulated with a single adder at the end. The number of adders increases logarithmically with the bit-width of the multiplier. Our design differs from prior work that uses racetrack in that it relies on a pipelined structure for implementing the design. The multiplicand will go through the pipeline bit by bit and accumulate with final results.
\end{comment}


Figure~\ref{Fig.:MAC} describes the multiplier we used for the MAC engine inside each PE. Both inputs and weights are strided across multiple racetracks, with one bit per track. This allows one value to be read per cycle. Our multiplier design is optimized to take advantage of the fact that the same LSTM cell input has to be multiplied with four different sets of weights. This allows a single decoder to be shared by four multipliers. The input value is decoded by the shared decoder, which determines what operations need to be performed on the weights. The same decoder output controls four sets of 1-bit adder clusters/trees. The entire multiplier is fully pipelined allowing multiplication of one input to four weights every cycle. The design enables high multiplication bandwidth in a very compact chip area footprint.

\begin{figure}
\centering
\includegraphics[width=0.7\linewidth,trim = 0 0 0 0 0]{figs/MAC2.pdf}
\caption{DWM-based multiplier.}\label{Fig.:MAC}
\vspace{-2em}
\end{figure} 
\begin{comment}
An interleaved multiplier has controllers which contain decoders for radix-4 booth algorithm. The multiplicand is within a single racetrack. Each controller modifies appropriate changes on the incoming bit of multiplicand and sends it the tree based structure of adders which are formed in a pipelines as is shown in Figure~\ref{Fig.:Adder}. Based on which segment of multiplier is the input of controllers, controllers injecting whether zero values or modified multiplicand incoming bit to the adders hierarchy. This multiplier is extensible to enable higher bits length by just duplicating the 8-bit multiplier and providing the adequate number of adders to the adder hierarchy. The final result is accumulated with a single adder at the end. The number of adders increases logarithmically with the bit-width of the multiplier. Our design differs from prior work that uses racetrack in that it relies on a pipelined structure for implementing the design. The multiplicand will go through the pipeline bit by bit and accumulate with final results.

The length of the pipeline is a function of input bit width.
Our deep pipeline will increase the throughput and efficiency of the multiplication
as it is a critical issue in neural networks consisting of LSTM cells.

Note that for maximum efficiency multipliers need to be bit-interleaved to access decoders in parallel. As in our design accelerator, the incoming data is bit interleaved across different racetracks we need to choose inputs as the multipliers and weights as multiplicands. Therefore we can keep weight in single racetrack non-interleaved. Secondly, due to the fact that in any LSTM cell each input is multiplied by 4 different sets of weights, using inputs as multiplier gives us the opportunity of controller sharing between four MAC engines in PEs. 
\end{comment}

\begin{comment}
\begin{figure}[b]
\centering
\includegraphics[width=0.75\linewidth,trim = 0 0 0 0 0]{figs/shift_controller.pdf}
\caption{LUT-based implementation of sigmoid/tanh.}\label{Fig.:LUT}
\vspace{-1em}
\end{figure}
\end{comment}


\begin{comment}
\subsection{Sensitivity to PE Configuration}

One of the design parameters we explore for RNNFast is the size of the basic compute unit, the PE. A larger PE reduces the number of LSTMs required to map a given neural network, reducing the network footprint and improving performance. On the other hand, a large number of weights in each PE increases decoding overhead and the latency
of each PE unit. Figure \ref{fig:sensitivity-performance} shows the execution time of multiple RNNFast designs with different PE sizes (16 to 1024 weights per PE) while maintaining the same total weights capacity. We show multiple neural network sizes ranging from 512 to 4K nodes. As the data shows, the configuration that yields the best performance across all network sizes is 2x512 which corresponds to a PE with 512 weights. 


Finding the best PE configuration is dependent on the pipeline latency. This means that we need to have a free PE to feed the input immediately when the input gets ready. According to our deep pipeline design, the latency of each pipeline stage is about single adder latency. This means that whenever a new input gets ready, one of 2 PEs is ready to get the data, and third PE is not needed anymore.
\end{comment}
\begin{comment}
\begin{figure}
\renewcommand{\baselinestretch}{1}
\centering
\includegraphics[width=0.8\linewidth]{figs/sensitivity-performance.pdf}
\caption{Performance sensitivity to the PE configuration (no.\
  PEs/LSTM $\times$ no.\ of weights/PE) for different
  neural network sizes.}
\label{fig:sensitivity-performance}
\vspace{-1em}
\end{figure}
\end{comment}



